Dynamic Matching: Reducing Integral Algorithms to Approximately-Maximal Fractional Algorithms

We present a simple randomized reduction from fully-dynamic integral matching algorithms to fully-dynamic "approximately-maximal" fractional matching algorithms. Applying this reduction to the recent fractional matching algorithm of Bhattacharya, Henzinger, and Nanongkai (SODA 2017), we obtain a novel result for the integral problem. Specifically, our main result is a randomized fully-dynamic $(2+\epsilon)$-approximate integral matching algorithm with small polylog worst-case update time. For the $(2+\epsilon)$-approximation regime only a \emph{fractional} fully-dynamic $(2+\epsilon)$-matching algorithm with worst-case polylog update time was previously known, due to Bhattacharya et al.~(SODA 2017). Our algorithm is the first algorithm that maintains approximate matchings with worst-case update time better than polynomial, for any constant approximation ratio. As a consequence, we also obtain the first constant-approximate worst-case polylogarithmic update time maximum weight matching algorithm.

==> better-polytime.tex <==
\section{Improved Deterministic Bounds}\label{sec:better-polytime}

In this section we briefly highlight how \Cref{lem:kernel-matching-number} implies a better approximation guarantee for the algorithms of \citet{bhattacharya2015deterministic}. We start by briefly describing the algorithms of \cite{bhattacharya2015deterministic}.

The algorithms of \cite{bhattacharya2015deterministic} dynamically maintain a $(1-\epsilon, d)$-kernel $H$ for some $d$, and a maximal matching or a matching with no augmenting paths of length less than $5$ in $H$. They prove that such matchings are respectively a $(4+O(\epsilon))$- and a $(3+O(\epsilon))$-approximation to the maximum matching in $G$. They further show how to maintain such matchings in worst-case (respectively, amortized) $O(d)$ update time.
However, by \Cref{lem:bounded-deg}, one can maintain a nearly-optimal matching in $H$ in essentially the same time (ignoring $\text{poly}(\epsilon^{-1})$ terms). Moreover, by \Cref{lem:kernel-matching-number}, such a $(1+\epsilon)$-approximate matching in $H$ is  $(2+O(\epsilon))$-approximate in $G$. These observations therefore immediately imply improved approximation ratios, given the kernel-maintenance of \citet{bhattacharya2015deterministic}, whose guarantees are given below.

\begin{lem}[Deterministic Kernel Maintenance \cite{bhattacharya2015deterministic}]\label{lem:det-kernel}
	There exist fully-dynamic algorithms for constructing a $(1-\epsilon, d)$-kernels 
	\begin{enumerate}
		\item for $d=O(\sqrt[3]{m}/\epsilon^2)$, in $O(d)$ worst-case update time, and
		\item for $d=O(\sqrt{n}/\epsilon)$, in $O(d)$ amortized update time.
	\end{enumerate}
\end{lem}


Given \Cref{lem:det-kernel} and \Cref{lem:bounded-deg}, and crucially \Cref{lem:kernel-matching-number}, we obtain the following.

\begin{thm}\label{thm:amortized-polytime}
	For all $\epsilon\leq \frac{1}{2}$, there exists a fully-dynamic $(2+O(\epsilon))$-matching algorithm with $O(\sqrt{n}/\epsilon^3)$ amortized update time.
\end{thm}

\begin{thm}\label{thm:wc-polytime}
	For all $\epsilon\leq \frac{1}{2}$, there exists a fully-dynamic $(2+O(\epsilon))$-matching algorithm with $O(\sqrt[3]{m}/\epsilon^4)$ worst-case update time.
\end{thm}

The proof of the above two theorems is immediate, but we present it here for completeness.
\begin{proof}[Proof (of Theorems \ref{thm:amortized-polytime} and \ref{thm:wc-polytime})]
	Running the algorithm of \Cref{lem:det-kernel}, maintain a $(1-\epsilon, d)$-kernel $H$ of $G$ (for the appropriate choice of $d$). The maintain a $(1+\epsilon)$-approximate matching in $H$, in time $O(d/\epsilon^2)$, using \Cref{lem:bounded-deg}. The update time follows. By \Cref{lem:kernel-matching-number}, the obtained matching is a $(2+O(\epsilon))$-approximation of the maximum matching in $G$.
\end{proof}

We note that the algorithm of Theorem \ref{thm:amortized-polytime} is superseded by the $O(\sqrt[4]{m}/\epsilon^{2.5})$ amortized update time algorithm of \citet{bernstein2016faster}, as $\sqrt[4]{m}\leq \sqrt{n}$ always. However, the algorithm of Theorem \ref{thm:wc-polytime} is an improvement on the current state of the art, yielding the current fastest deterministic fully-dynamic matching algorithm with worst-case update time (ignoring $\text{poly}(\epsilon^{-1})$ terms), showing this update time allows for maintenance of a $(2+\epsilon)$-approximate matching.

